An\'alise de ambiguidade lingu\'istica em modelos de linguagem de grande escala (LLMs)

Linguistic ambiguity continues to represent a significant challenge for natural language processing (NLP) systems, notwithstanding the advancements in architectures such as Transformers and BERT. Inspired by the recent success of instructional models like ChatGPT and Gemini (In 2023, the artificial intelligence was called Bard.), this study aims to analyze and discuss linguistic ambiguity within these models, focusing on three types prevalent in Brazilian Portuguese: semantic, syntactic, and lexical ambiguity. We create a corpus comprising 120 sentences, both ambiguous and unambiguous, for classification, explanation, and disambiguation. The models capability to generate ambiguous sentences was also explored by soliciting sets of sentences for each type of ambiguity. The results underwent qualitative analysis, drawing on recognized linguistic references, and quantitative assessment based on the accuracy of the responses obtained. It was evidenced that even the most sophisticated models, such as ChatGPT and Gemini, exhibit errors and deficiencies in their responses, with explanations often providing inconsistent. Furthermore, the accuracy peaked at 49.58 percent, indicating the need for descriptive studies for supervised learning.

==> sections/backlog_respostas.tex <==
\subsection{Os modelos de linguagem conseguem delimitar e explicar corretamente a origem da ambiguidade nas frases testadas? A explicação dada é coerente com a classificação da ambiguidade feita pelo modelo?}\label{resultados-q-2}

O ChatGPT, na maior parte dos testes com frases de ambiguidade léxica e sintática, conseguiu explicar corretamente qual elemento das sentenças que gera a ambiguidade, mesmo que a classificação do tipo de ambiguidade não estivesse adequada. Por exemplo, em “Isso não é legal!”, o modelo justificou a classificação como ambiguidade lexical, pois a palavra “legal” pode ser interpretada tanto no sentido de “permitido”, como no sentido “incrível” ou “ótimo”.

No entanto, o modelo, por vezes, apresentou explicações pouco prováveis para justificar a ambiguidade presente nas frases. Em “Eu gosto de damas, são tão educadas”, o ChatGPT disse, inicialmente, que não sabia dizer se a frase era ambígua e, no Experimento 2, a classificou como ambiguidade sintática, entendendo que “damas” pode se relacionar tanto a “são educadas” como a “gosto de”. A análise sintática feita pelo modelo não faz sentido porque o que ele afirma não são aspectos excludentes: “damas” refere-se tanto a “são educadas” quanto a “gosto de”.

Em relação às frases de ambiguidade semântica, o ChatGPT não identificou esse tipo de ambiguidade em nenhuma delas, sugerindo ambiguidades de escopo, possessivos e anexação. De maneira oposta, a Bard apresentou a tendência de classificar sentenças de ambiguidade léxica e semântica como tendo ambiguidade semântica e, nas frases de ambiguidade sintática, foi indicada a ambiguidade referencial em grande parte dos testes, o que está relacionado com a sintaxe. 

A Bard, assim como o ChatGPT, na maioria das vezes, identificou qual elemento das sentenças que gera a ambiguidade, mas também apresentou algumas explicações inusitadas. No caso da frase "Abandonei meu irmão contrariado", a Bard justificou que a frase contém ambiguidade semântica pela palavra "contrariado" ter dois significados diferentes: "zangado ou decepcionado" ou "ter um desejo ou vontade forte de fazer algo". Assim, o modelo não identificou a ambiguidade sintática que, de fato, ocorre, dado que contrariado pode estar relacionado tanto ao sujeito da frase "eu", o qual está implícito, quanto ao objeto "irmão".



\subsubsection{Ambiguidade Léxica}
Como cada sentença dos experimentos de um a três continham um tipo de ambiguidade nos subtipos — homofonia e homonímia real ou polissemia (cuja distinção não será aqui explorada por questões de indiferença prática) — da lexical, é importante entender cada um a fim de melhor compreender como e em quais aspectos as IAs falham na missão de desambiguá-las. As frases com homofonia eram:
\begin{enumerate}
    \item Sabe como chama a sorveteria do Michel Teló? Ice te pego.
    \item Qual o contrário de papelada? Pá vestida.
    \item Viajem!
    \item Sabe por que não seria bom um filme só sobre números? Porque seria uma má temática.
    \item Sabe por que um homem estava com a orelha encostada na pedra? Porque ele estava ouvindo arrocha.
    \item Acende logo!
\end{enumerate}

Em todas essas, a palavra fonológica \cite{ulrich2016diferentes} se confunde com possibilidades de palavras gráficas (ibidem), tal qual se visualiza na tabela \ref{tab:correspondência}, cuja organização é respectiva à enumeração acima.
\begin{table}[h]
\caption{Correspondência entre as palavras fonológica e gráfica}
\label{tab:correspondência}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
{[}\textipa{"aj.si}{]}                                                                                         & {[}\textipa{""pa.pe."la.d5}{]}                                                                                            & {[}\textipa{vi.a.Z\~{e}\~{j}}{]}                                                                             & {[}\textipa{ma.te."ma.tSi.k5}{]}                                                                                            & {[}\textipa{a.hO.S5}{]}                                                                                           & {[}\textipa{a.s\~{e}\~{j}.dI}{]}                                                                               \\ \hline
\begin{tabular}[c]{@{}l@{}}\textless{}ai se\textgreater\\ \textless{}ice\textgreater{}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textless{}papelada\textgreater\\ \textless{}pá pelada\textgreater{}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textless{}viajem\textgreater\\ \textless{}viagem\textgreater{}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textless{}má temática\textgreater\\ \textless{}matemática\textgreater{}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textless{}arrocha\textgreater\\ \textless{}a rocha\textgreater{}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textless{}acende\textgreater\\ \textless{}ascende\textgreater{}\end{tabular} \\ \hline
\end{tabular}
\source{Própria.}
\end{table}
\begin{table}[ht]
Visão geral dos resultados do ChatGPT:
    \centering
    \begin{tabular}{|l|l|l|l|}
    \hline
        (D/ND)E & (D/ND)PE & (D/ND)C & (D/ND)SE\\
    \hline
       12 & 8 & 15 & 5\\
    \hline
    \end{tabular}
    \caption{Classificação das respostas do ChatGPT}
    \label{tab:GPT}

Legenda:
\begin{enumerate}
    \item D desambigou
    \item ND não desambigou
    \item E explicação errada
    \item C explicação correta
    \item PE parcialmente errada
    \item SE sem explicação
\end{enumerate}
\end{table}

O ChatGPT desambigou corretamente (apesar de certas inconsistências) as frases em 9 dos 14 testes realizados, de modo a apresentar aproximadamente 64\% de sucesso (9/14)\footnote{Não é esse nenhum dos parâmetros consensuais de análise de modelo de linguagem, por isso "sucesso" não deve ser entendido como um termo técnico, senão como um elemento didático do qual se apropriou os autores}. Apesar de tal êxito, nos casos em que a desambiguação foi corretamente feita, houve confusão entre as possibilidades gráficas e, ademais, o chat não indicou, em nenhum momento, as duas possibilidades de interpretação de forma completamente consistente devido à exata confusão entre as formas escritas.

Nos contextos nos quais não houve desambiguação, identifica-se a explicação cuja preponderância na resposta não responde à expectativa de concreta desambiguação, visto haver uma incoerência entre a pesquisa e o retrucamento fornecido, os quais não se coincidem, tal qual ocorreu nas demais frases da seção das quatro erradas.

Dessa forma, em uma ocorrência, fez-se uma confusão com a língua inglesa, talvez pela IA em questão haver sido lançada inicialmente para um público nesse idioma. Nos outros casos, no lugar de se executar a desambiguação das sentenças, houve, majoritariamente, sua devida explanação, isto é, explicou-se o porquê de a ambiguidade estar presente. Situação essa que pode ser remetida a problemas na enunciação dos comandos por trabalhos passados na área com questões semelhantes, como em \textcite{ortega2023linguistic}.

Por outro lado, nas outras 26 frases de homonímia real/polissemia, 12 foram desambiguadas propriamente, situação na qual se pode analisar o porquê da predominância de erros (os 14 restantes). Alguns desses (4) correspondem à incongruência entre o comando e o dado, tal qual ocorreu na seção de homófonos. Destarte, pode-se dizer que a acurácia de inteligibilidade ((D/ND)C) do chat foi de aproximadamente 61\% (16/26), visto que o entendimento em si foi correto, embora o comando não tenha sido atendido satisfatoriamente.

Nesse sentido, restam os 10 casos nos quais nem o comando, nem a inteligibilidade do conceito, foram atendidos satisfatoriamente. Nesses casos, em função de duas frases apresentarem construções sintáticas semelhantes, o erro mais comum foi quanto ao paralelismo das frases. Apresentam-se os exemplos a seguir:
\begin{enumerate}
    \item João foi à mangueira, assim como Maria.
    \item João quer mangas, assim como Maria.
\end{enumerate}
Em 1, “mangueira” pode ser tanto a mangueira de água, por exemplo, como a árvore, em ambas as orações. Dessa forma, teoricamente haveria quatro interpretações, uma em que João foi à mangueira de água e Maria foi à mesma; uma em que João foi à árvore "mangueira" e Maria foi à mesma; outra em que João foi à mangueira de água e Maria, à árvore, e vice-versa. Entretanto, aos falantes, só as duas primeiras interpretações são possíveis, porquanto, se João foi à mangueira de água, Maria foi à mesma, consequentemente, pelo paralelismo existente entre as orações.

Todavia, a IA oferece uma interpretação não prevista em estudos teóricos anteriores sobre ambiguidade, a exemplo de \cite{kroeger2023analyzing}, a de que Maria foi a um lugar diferente ou quer algo distinto a João, que não nenhum dos significados dos significantes homônimos. Como a ambiguidade identificada foi na estrutura e não na palavra das orações, conclui-se ser um problema de reconhecimento sintático. Tal empecilho não o é a um ser humano pela distinção que ocorre na aquisição de linguagem por máquinas em contraposição a seres humanos, isto é, o uso de estatística e árvores sintáticas\footnote{"Árvores sintáticas" não no sentido estritamente gerativista, senão nas tradições acadêmicas mais recentes. Aqui, não se fará uma discussão mais aprofundada sobre esse conceito na aquisição por não ser esse o objetivo do presente artigo.}, respectivamente.

Outro erro semlhante foi o apresentado em "Pedi um prato ao garçom.". Nesse, embora a sintaxe não funcione da mesma forma que as erratas das frases com "assim como", a identificação desse tipo de ambigudade foi incorretamente apontado também. Pela resposta, ficar-se-ia em dúvida se a incoerência decorre da equivalente confusão, mas, em "A ambiguidade ocorre devido à falta de clareza na estrutura da frase, o que permite essas diferentes interpretações.", fica claro o equívoco e seu motivo: a falta de capacidade de interpretação dos processos de ligação sintagmática dos modelos estudados em função da distinção de como ocorre a aquisição de linguagem por máquinas e seres humanos. Tal asseveração advoca em prol de distinções contrastantes e constantes em ambas.

Por fim, outras vicissitudes de menor frequência foram: identificação indevida de outra ambiguidade, mas com lógica coerente; interpretações pragmáticas não intentadas, coerentemente explanadas em maioria, a partir de figuras de linguagem; e a afirmação de falta de dados suficientes à execução da tarefa.

No que tange à Bard, sempre há identificação de ambiguidade, seja um verdadeiro, seja um falso positivo. Logo, percebe-se, inicialmente, a inexistente especificidade, isto é, de distinguir o que não é ambiguidade e, portanto, o que o é também, embora a sensibilidade seja teoricamente alta, visto que o modelo sempre responde "sim" no primeiro experimento. Ademais, na maioria dos testes realizados, fala-se estar presente ambiguidade semântica. Diante de tais deficiências, analisam-se as desambiguações, cuja execução é diretamente afetada pelas tendências padrões das perguntas anteriores (experimentos um e dois).

Em 40 dos casos, as explicações da Bard foram da seguinte forma classificadas, cuja legenda é a mesma seguida nos resultados da ChatGPT:

\begin{table}[ht]
    \centering
    \begin{tabular}{|l|l|l|l|}
    \hline
        (D/ND)E & (D/ND)PE & (D/ND)C & (D/ND)SE\\
    \hline
       13 & 17 & 8 & 2\\
    \hline
    \end{tabular}
    \caption{Classificação das respostas da Bard}
    \label{tab:Bard}
\end{table}

A partir de tais dados, vê-se, inicialmente, que a Bard não apresentou qualquer identificação de homofonia. Tal conclusão é observável em razão de as frases que apresentaram homofonia terem sido erroneamente explicadas. O modelo analisa a palavra gráfica, mas não a relaciona foneticamente a nenhuma outra em nenhum dos casos. Mesmo naqueles em que houve acerto parcial (os mesmos de erro parcial), os termos focados na explanação foram aqueles identificáveis pela escrita, enquanto seus homófonos passaram despercebidos em relação à Bard, o que não ocorreu com o ChatGPT, o qual possui essa capacidade, mesmo não possuindo as transcrições e ou a pronunciação das palavras.

Destarte, é inferível que o Chat utiliza alguma competência que dispensa esses requerimentos, ao menos nos casos selecionados, o que pode ser mais explorado em estudos futuros. A Bard, por sua vez, não detém o arcabouço necessário a tal tipo de identificação, de modo a não perceber fenômenos no nível fonético.

No caso das homonímias reais, a Bard apresenta mais facilidade de identificação e explicação que nos casos de homofonia, tanto o é que as explicações corretas estão todas naquelas. Por outro lado, ainda predominaram-se as justificativas equivocadas. O primeiro teste a empregar uma homonímia foi o do trocadilho "Sabe o que aconteceu com o lápis quando soube que o papel acabou? Ficou desapontado.", no qual o modelo apontou somente um dos significados ao significante "desapontado", sendo o sentido mais convencional de "Que sentiu desapontamento; decepcionado, desiludido."\footnote{Retirado do dicionário online Michaelis.}, embora o significado de "estar sem ponta" também estivesse presente, de modo a enfraquecer a hipótese da falta de dicionarização.

No segundo teste de homonímia real, a frase "Como o padre bateu o carro? Dando uma rezinha." só chamou a atenção do modelo para "rezinha" como o diminutivo de "ré". Os significados adjacentes os quais ascenderiam ambiguidade foram diferentes nas duas vezes em que foram rodados os testes e não se encontraram base teórica a esses, então não se revelam de tão grande importância. Nesse caso, ambos os significados são dicionarizados\footnote{A exemplo da Infopédia.}, mas não houve abordagem de ambos.

A partir de tal incapacidade explicativa da hipótese da dicionarização, surgem outras possibilidades explicativas a serem exploradas por estudos ulteriores, sejam:
\begin{enumerate}
    \item Frequência;
    \item data de entrada na língua;
    \item data de entrada no dicionário.
    \item contexto
\end{enumerate}
Outrossim, um ponto de convergência em relação ao ChatGPT é a dificuldade com as estruturas sintáticas típicas do português, a exemplo dos casos de paralelismo em "João foi à mangueira, assim como Maria." e "João quer mangas, assim como Maria.". Não só isso, mas também explicações aludindo figuras de linguagem, como no Chat.

Por fim, outros erros comuns foram incluir significados de palavras que só o teriam em expressões idiomáticas e entender a sentença como uma verdade universal no mundo cuja concretude levaria à explicação, de modo a não fornecer a explicação à ambiguidade, um dos casos de "SE". Dessa forma, os erros de ambos os modelos são mapeados tal qual demonstra a tabela \ref{tab:BardChat}.

\begin{table}[ht]
    \centering
    \begin{tabular}{|l|l|l|l|}
    \hline
        Níveis linguísticos & Tipo de erro & ChatGPT & Bard\\
    \hline
     \multirow{2}{*}{sintaxe} & EP & 4 & 3\\
  \cline{2-4}
  & TV & 2 & 0\\
    \hline
       \multirow{2}{*}{semântica} & OS & 2 & 2\\
  \cline{2-4}
  & 1S & 5 & 10\\
    \hline
       \multirow{2}{*}{lexicologia} & OA & 3 & 3\\
  \cline{2-4}
  & CG & 1 & 0\\
    \hline
       \multirow{2}{*}{estilística} & FL & 1 & 0\\
  \cline{2-4}
  & IF & 0 & 5\\
    \hline
        \multirow{2}{*}{pragmática} & V & 1 & 5\\
  \cline{2-4}
  & CL & 1 & 0\\
    \hline
    \end{tabular}
    \caption{Análise geral dos modelos}
    \label{tab:BardChat}
\end{table}

\begin{enumerate}
\item Legenda:
\item CL confusão entre línguas
\item OA outra ambiguidade
\item OS outro sentido
\item EP erro de paralelismo
\item 1S um significado
\item CG confusão gráfica
\item FL figura de linguagem
\item V vaguidão
\item TV transitividade verbal
\item IF intensão do falante
\end{enumerate}

Na legenda acima, faz-se necessário algumas considerações. Na vaguidão, o modelo analisa a indeterminação semântica ao invés de uma ambiguidade em si. Entretanto, como a análise fornecida pela IA era baseada nos usos que a frase poderia assumir, foi essa categorizada em "pragmática". Em "intensão do falante", explanou-se os contextos prosódicos os quais poderiam distinguir uma pergunta de uma assertiva, por exemplo. As outras categorizações foram nomeadamente exploradas e, de qualquer maneira, entende-se a tebela como um resumo das justificativas dessa seção. Ademais, (D/ND)SE ou (D/ND)C não foram consideradas ao gráfico em função de não possuírem explicação ou erro os quais devessem enquadrar-se em alguma categoria.
\subsubsection{Ambiguidade Sintática}

Na terceira etapa, a desambiguação das orações feita pela Bard e ChatGPT demonstraram certa imprecisão em alguns casos, porque no geral as análises apresentadas estavam incorretas e os critérios usados nas frases classificadas com ambiguidade sintática também, pendendo para uma abordagem semântica, lexical ou voltada para a necessidade de um contexto favorável para desambiguar as sentenças. Temos, por exemplo, o caso da frase “A minha mãe brava perguntou que horas eu cheguei.”, avaliada pela Bard com ambiguidade de causa no primeiro teste e com ambiguidade semântica no segundo. Em ambos os casos, a inteligência afirma que a razão pela irritação da mãe não está clara e deveria haver mais contexto para entender se ela estava brava pelo atraso do filho ou por algum outro motivo, porém em nenhuma análise consta que o item acessório “brava” pode ser um adjunto adverbial ou adnominal, causando a ambiguidade sintática por não saber se o termo se refere ao verbo ou ao sujeito e, nesse caso, se estaria tendo a função de restringir ou explicar. 

Posteriormente, um caso semelhante ocorre na sentença “Carlos observou Tiago malhando” em que novamente a Bard recorre à classificação de ambiguidade semântica e explica que “É importante fornecer mais informações sobre o contexto da situação para poder determinar qual é o significado pretendido da palavra ‘observou’, tendo em vista que essa palavra poderia indicar que Carlos estava vendo Tiago ou que Carlos examinou Tiago, porém, não é discutida a ambiguidade sintática presente na palavra malhando, que pode exercer a função de adjunto adnominal do objeto da frase, que é Tiago, ou poderia ser um adjunto adverbial do verbo “observar”, transmitindo a ideia de que Carlos, enquanto estava malhando, observou Tiago.

Também temos o caso da sentença ambígua “Pedro me mandou um cartão postal de Veneza”, uma vez que o adjunto “de Veneza” pode referir-se ao local em que Pedro estava ou à imagem presente no cartão postal. Aqui, a ChatGPT a caracterizou com ambiguidade sintática, mas cometeu um equívoco ao definir que a ambiguidade se dá devido ao pronome “me”. Isto é, Pedro poderia ter enviado um cartão ao locutor da frase ou para uma terceira pessoa que repassou o cartão. A segunda vez em que é questionada, afirma novamente que há ambiguidade, caracterizando-a como uma ambiguidade de regência verbal devido ao pronome “me”. Quando é solicitado que ela realize a desambiguação da frase, a ChatGPT apresenta a frase "Pedro me mandou um cartão postal de Veneza”, que é precisamente idêntica a frase fornecida e, na tentativa de solucionar a ambiguidade, a inteligência apresenta a sentença "Pedro mandou um cartão postal de Veneza para a minha amiga Maria, e ela me mostrou o cartão", mas a ambiguidade no adjunto “de Veneza” permanece e por fim, outra solução proposta é mudar a alocação do pronome: Pedro mandou um cartão postal de Veneza para mim, mantendo a frase ambígua. 

Outra frase com ambiguidade que foi analisada de forma errada é “Policial prende criminoso com arma de brincadeira”, a ambiguidade sintática reside no adjunto “de brincadeira”, que pode ser compreendido de quatro maneiras distintas: o policial portava uma arma de brincadeira no momento da prisão (1); o criminoso estava com uma arma de brincadeira quando foi detido (2); de brincadeira, o policial prendeu o criminoso que estava armado (3); de brincadeira, o policial armado prendeu um criminoso (4). As análises sintáticas em questão são:

[Policial [prende [criminoso com arma de brincadeira]]]

[Policial com arma de brincadeira [prende [criminoso]]]

[Policial [prende [criminoso com arma [de brincadeira]]]]

[Policial com arma [prende [criminoso [de brincadeira]]]]

A ChatGPT identifica uma ambiguidade lexical, atribuindo essa ocorrência ao substantivo “arma”, determinando que ela pode ser compreendida como uma arma de verdade ou não. No segundo momento, a ChatGPT responde que não sabe definir se o período é ou não ambíguo, explicando que a ambiguidade se dá através do contexto que a frase foi empregada, e por não obter essa informação, não é capaz de responder. No entanto, ao desambiguar a frase, ela apresenta as opções: "Policial prende criminoso com arma de brincadeira de plástico." e  "Policial prende criminoso que portava uma arma de brincadeira.", em que a primeira seria uma desambiguação com contexto e a segunda, com complemento. Aqui, ambas as soluções apresentadas não visam a ambiguidade sintática no sentido de que os adjuntos permanecem com sentido ambíguo. 

A confusão em reconhecer ambiguidade nos itens lexicais no lugar da ambiguidade sintática apareceu em muitos testes e em ambas as inteligências artificiais. Temos o caso, por exemplo, da frase sem ambiguidade “A filha ligou para a mãe no momento do acidente de carro”, em que a ChatGPT classificou como tendo “ambiguidade temporal” a partir da explicação que esse tipo de ambiguidade aparece em orações em que não está explícito o período de tempo da ação, logo, poderia ser interpretado que a filha ligou no exato momento do acidente ou em um momento próximo a esse evento. A Bard analisou de forma semelhante, mesmo tendo classificando a frase com ambiguidade sintática, dizendo que “a palavra ‘momento’ pode ser interpretada de duas maneiras: o momento exato em que o acidente aconteceu ou um período de tempo mais longo que inclui o momento do acidente. Para desambiguar a frase, precisamos saber mais sobre a situação.” Assim, nota-se que tanto a ChatGPT como a Bard têm dificuldade em reconhecer a ambiguidade sintática e analisar corretamente suas causas por meio dos constituintes da frase. 



\subsubsection{Ambiguidade Semântica}

No Experimento III, na maior parte dos testes, ambos os modelos de linguagem sugeriram frases adequadas para a desambiguação das sentenças com ambiguidade semântica, sempre destacando a importância do contexto para a interpretação das frases. Esse é um ponto-chave quando trata-se de ambiguidade, especialmente no caso da ambiguidade semântica, pois, na maioria das vezes, as frases não estão abertas à ambiguidade quando estão situadas em contextos de produção específicos. É o caso da ambiguidade semântica causada por pronomes, como em "Ela não gosta da amiga dela". Tal frase, descontextualizada, é ambígua, mas, quando usada em um conversa em que está claro a quem se refere ao usar "ela" e "dela", não há dúvidas sobre os referentes. Um exemplo disso foi visto com a frase "Ana me contou um segredo sobre ela", em que o ChatGPT propôs a desambiguação esperada, compreendendo que "ela" pode se referir tanto à Ana, quanto a uma outra pessoa.

Entretanto, houve 7 casos em que as respostas do ChatGPT foram inesperadas. Em “Ele saiu da loja de carro”, uma das sugestões para eliminar a ambiguidade foi reescrever o enunciado como: “Ele saiu da loja, e o carro estava estacionado do lado de fora.”, porque, assim, “deixamos claro que a pessoa saiu a pé, e o carro estava estacionado do lado de fora da loja”, segundo o modelo de linguagem, o que vai além dos sentidos possíveis na sentença original. Outro caso inusitado ocorreu com a frase “Ele não sabia que era o dia do seu aniversário”, visto que uma das desambiguações indicadas pelo ChatGPT foi: “Ele sabia que era o dia do seu aniversário, mas não sabia disso", demonstrando uma clara contradição. Também é válido citar o ocorrido na frase "Ela estava perto da mangueira", em que o ChatGPT, em um dos testes, trouxe como possibilidades de sentido "Ele estava em uma posição física próxima à mangueira" e "Ele estava envolvido na operação ou manipulação da mangueira". Aqui, não foi identificado a ambiguidade da palavra "mangueira", que pode se referir à àrvore ou ao objeto destinado a conduzir líquidos.

Em relação às respostas do Bard, no Experimento III, a maioria das respostas foi apropriada, como em "Paulo não entrou na universidade de novo", na qual o modelo de linguagem indicou que possíveis reescritas da sentença que eliminam a ambiguidade são "Paulo não foi aceito na universidade de novo" e "Paulo não entrou na universidade de novo depois de ter se formado", por exemplo. Todavia, 6 respostas trouxeram ideias fora do esperado. Na frase “Ela não gosta da amiga dela”, o Bard recomendou adicionar mais informações para esclarecer o motivo dela não gostar da amiga, ao invés de fazer a desambiguação sobre os referentes, sugerindo as frases: “Ela não gosta da amiga dela porque a amiga dela é falsa” e “Ela não gosta da amiga dela porque a amiga dela é egoísta”, por exemplo. Em outro caso, na sentença “A carteira foi danificada”, o Bard também sugeriu opções que especificassem informações não necessariamente ambíguas, visto que ele interpretou que a ambiguidade estaria em “danificado”, assim, deveria ser especificado se “A “carteira foi danificada fisicamente” ou “A carteira foi danificada financeiramente”. Tais casos demonstram interpretações que, dificilmente, seriam feitas por falantes de língua portuguesa.

Dado o exposto, entende-se que ambos os modelos de linguagem conseguem propor desambiguações adequadas para as frases, ainda que casos com interpretações inesperadas aconteçam. As frases expostas apresentam ideias, significativamente, distantes entre si, por isso, não foi possível identificar um padrão que possa motivar uma interpretação equivocada.

No que diz respeito às frases sem ambiguidade, vale a análise das sentenças em que a resposta do modelo foi diferente nas coletas. Na primeira coleta da sentença "Ela não gosta daquela mulher", a ChatGPT respondeu que a frase não era ambígua e que "possui apenas uma interpretação direta e clara". No Experimento 3, contudo, ela pede desculpas e afirma que "a ambiguidade surge da falta de informações claras sobre quem é o sujeito "ela" e a relação entre "aquela mulher" e o contexto geral da conversa". Na segunda coleta, ela já identifica a ambiguidade no primeiro experimento e, quando perguntada sobre o tipo, responde que é uma ambiguidade de escopo, já que a posição da palavra "não" pode gerar interpretações diferentes em relação ao que está sendo negado, na sua avaliação. A Bard, por sua vez, apontou ambiguidade sintática devido ao fato de que não é possível reconhecer qual o sujeito e o objeto da frase. Na coleta seguite, afirmou que há uma ambiguidade semântica porque o verbo "gostar" pode ter vários significados.

Na sentença "Ela estava doente e avisou o chefe", a ChatGPT inicialmente disse que não havia ambiguidade. Contudo, já no segundo experimento, ela identificou uma ambiguidade de coordenação e sugere reformulações na coordenação utilizando os conectivos "em seguida" ou "ao mesmo tempo". Na outra coleta, ela identifica ambiguidade e afirma que é estrutural, pois gera interpretações diferentes acerca de quem avisou o chefe. A Bard, inicialmente, indicou que "a palavra "avisou" pode ser interpretada como "comunicar algo a alguém" ou "dar uma advertência a alguém" e, por isso, a frase é ambígua. Em seguida, na segunda coleta, afirmou que existe uma ambiguidade de referência, uma vez que "chefe" pode ser tanto o chefe imediato quanto o chefe geral.

A análise sentença "Gostamos da cor rosa" merece destaque porque o modelo da OpenAI respondeu "não sei" nas duas coletas do Experimento 1. No Experimento 2, o modelo dá explicações confusas quanto ao tipo de ambiguidade. Na primeira coleta, afirma que "a sentença pode significar que a pessoa gosta da cor rosa em geral" e, na segunda, aponta uma possível confusão entre a flor e a cor, além de uma ambiguidade de escopo em que "não ficaria claro se estão compartilhando uma preferência pessoal ou se estão fazendo uma observação geral sobre a cor rosa". Pode-se perceber que o modelo tende a superinterpretar a frase, encontrando ambiguidades sem nexo. Para a Bard, a ambiguidade se encontra no fato de que "nós" pode se referir a um conjunto de diferentes pessoas.










==> sections/internationalization.tex <==
% AND
\DeclareTranslation{Portuguese}{and}{e}
\DeclareTranslation{English}{and}{and}
\DeclareTranslation{Spanish}{and}{y}
\DeclareTranslation{French}{and}{et}
\DeclareTranslation{German}{and}{und}
% SESSION
\DeclareTranslation{Portuguese}{session}{Seção}
\DeclareTranslation{English}{session}{Session}
\DeclareTranslation{Spanish}{session}{Sección}
\DeclareTranslation{French}{session}{Section}
\DeclareTranslation{German}{session}{Sektion}
% SESSION NAME - BEGIN
% article
\DeclareTranslation{Portuguese}{articles}{Artigos}
\DeclareTranslation{English}{articles}{Articles}
\DeclareTranslation{Spanish}{articles}{Artículos}
\DeclareTranslation{French}{articles}{Articles}
\DeclareTranslation{German}{articles}{Artikel}
% dossier
\DeclareTranslation{Portuguese}{dossier}{Dossiê}
\DeclareTranslation{English}{dossier}{Dossier}
\DeclareTranslation{Spanish}{dossier}{Dosier}
\DeclareTranslation{French}{dossier}{Dossier}
\DeclareTranslation{German}{dossier}{Dossier}
% reports
\DeclareTranslation{Portuguese}{reports}{Relatos de experiência}
\DeclareTranslation{English}{reports}{Experience reports}
\DeclareTranslation{Spanish}{reports}{Relatos de experiencia}
\DeclareTranslation{French}{reports}{Rapports d'expérience}
\DeclareTranslation{German}{reports}{Erfahrungsberichte}
% essays
\DeclareTranslation{Portuguese}{essays}{Ensaios}
\DeclareTranslation{English}{essays}{Essays}
\DeclareTranslation{Spanish}{essays}{Ensayos}
\DeclareTranslation{French}{essays}{Essais}
\DeclareTranslation{German}{essays}{Aufsätze}
% reviews
\DeclareTranslation{Portuguese}{reviews}{Resenhas críticas}
\DeclareTranslation{English}{reviews}{Critical reviews}
\DeclareTranslation{Spanish}{reviews}{Reseñas críticas}
\DeclareTranslation{French}{reviews}{Recensions de livre}
\DeclareTranslation{German}{reviews}{Kritische Rezensionen}
% interviews
\DeclareTranslation{Portuguese}{interviews}{Entrevistas}
\DeclareTranslation{English}{interviews}{Interviews}
\DeclareTranslation{Spanish}{interviews}{Entrevistas}
\DeclareTranslation{French}{interviews}{Entretiens}
\DeclareTranslation{German}{interviews}{Interview}
% editorial
\DeclareTranslation{Portuguese}{editorial}{Editorial}
\DeclareTranslation{English}{editorial}{Editorial}
\DeclareTranslation{Spanish}{editorial}{Editorial}
\DeclareTranslation{French}{editorial}{Éditorial}
\DeclareTranslation{German}{editorial}{Leitartikel}
% SESSION NAME - END
% CORRESPONDING AUTHOR
\DeclareTranslation{Portuguese}{correspondingauthor}{Autor Correspondente}
\DeclareTranslation{English}{correspondingauthor}{Corresponding author}
\DeclareTranslation{Spanish}{correspondingauthor}{Autor correspondiente}
\DeclareTranslation{French}{correspondingauthor}{Autor correspondiente}
\DeclareTranslation{German}{correspondingauthor}{Entsprechender Autor}
% EDITED BY
\DeclareTranslation{Portuguese}{editedby}{Editado por}
\DeclareTranslation{English}{editedby}{Edited by}
\DeclareTranslation{Spanish}{editedby}{Editado por}
\DeclareTranslation{French}{editedby}{Édité par}
\DeclareTranslation{German}{editedby}{Bearbeitet von}
% SECTION EDITOR
\DeclareTranslation{Portuguese}{sectioneditor}{Editor de seção}
\DeclareTranslation{English}{sectioneditor}{Section Editor}
\DeclareTranslation{Spanish}{sectioneditor}{Editor de sección}
\DeclareTranslation{French}{sectioneditor}{Editeur de section}
\DeclareTranslation{German}{sectioneditor}{Abschnittseditor}
% LAYOUT EDITOR
\DeclareTranslation{Portuguese}{layouteditor}{Editor de layout}
\DeclareTranslation{English}{layouteditor}{Layout editor}
\DeclareTranslation{Spanish}{layouteditor}{Editor de maquetación}
\DeclareTranslation{French}{layouteditor}{Éditeur de mise en page}
\DeclareTranslation{German}{layouteditor}{Layout-Editor}
% RECEIVED
\DeclareTranslation{Portuguese}{received}{Recebido em}
\DeclareTranslation{English}{received}{Received on}
\DeclareTranslation{Spanish}{received}{Recibido el}
\DeclareTranslation{French}{received}{Reçu en}
\DeclareTranslation{German}{received}{Empfangsdatum}
% ACCEPTED
\DeclareTranslation{Portuguese}{accepted}{Aceito em}
\DeclareTranslation{English}{accepted}{Accepted on}
\DeclareTranslation{Spanish}{accepted}{Aceptado el}
\DeclareTranslation{French}{accepted}{Acceptée en}
\DeclareTranslation{German}{accepted}{Akzeptiertes Datum}
% PUBLISHED 
\DeclareTranslation{Portuguese}{published}{Publicado em}
\DeclareTranslation{English}{published}{Published on}
\DeclareTranslation{Spanish}{published}{Publicado el}
\DeclareTranslation{French}{published}{Publication en}
\DeclareTranslation{German}{published}{Veröffentlichungsdatum}
% LICENSE - requires: doclicense
\DeclareTranslation{Portuguese}{license}{\makeatletter\input{doclicense-brazilian.ldf}\makeatother\doclicenseText\\\doclicenseIcon}
\DeclareTranslation{English}{license}{\makeatletter\input{doclicense-english.ldf}\makeatother\doclicenseText\\\doclicenseIcon}
\DeclareTranslation{Spanish}{license}{\makeatletter\input{doclicense-spanish.ldf}\makeatother\doclicenseText\\\doclicenseIcon}
\DeclareTranslation{French}{license}{\makeatletter\input{doclicense-french.ldf}\makeatother\doclicenseText\\\doclicenseIcon}
\DeclareTranslation{German}{license}{\makeatletter\input{doclicense-german.ldf}\makeatother\doclicenseText\\\doclicenseIcon}
% KEYWORD
\DeclareTranslation{Portuguese}{keywords}{Palavras-chave}
\DeclareTranslation{English}{keywords}{Keywords}
\DeclareTranslation{Spanish}{keywords}{Palabras clave}
\DeclareTranslation{French}{keywords}{Mots-cl\'{e}s}
\DeclareTranslation{German}{keywords}{Schl\"{u}sselw\"{o}rter}
% Authors contributions BEGIN
% AUTHOR CONTR.
\DeclareTranslation{Portuguese}{authorcontributions}{Contribuições dos autores}
\DeclareTranslation{English}{authorcontributions}{Author contributions}
\DeclareTranslation{Spanish}{authorcontributions}{Contribuciones de los autores}
\DeclareTranslation{French}{authorcontributions}{Les conttributions des auteurs}
\DeclareTranslation{German}{authorcontributions}{Autorenbeiträge}
% CONCEPTUALIZATION 
\DeclareTranslation{Portuguese}{conceptualization}{Conceituação}
\DeclareTranslation{English}{conceptualization}{Conceptualization}
\DeclareTranslation{Spanish}{conceptualization}{Conceptualización}
\DeclareTranslation{French}{conceptualization}{Conceptualisation}
\DeclareTranslation{German}{conceptualization}{Konzeptualisierung}
% DATA CURATION
\DeclareTranslation{Portuguese}{datacuration}{Curadoria de dados}
\DeclareTranslation{English}{datacuration}{Data curation}
\DeclareTranslation{Spanish}{datacuration}{Curación de datos}
\DeclareTranslation{French}{datacuration}{Conservation des données}
\DeclareTranslation{German}{datacuration}{Daten-Kuration}
% FORMAL ANALYSIS
\DeclareTranslation{Portuguese}{formalanalysis}{Análise formal}
\DeclareTranslation{English}{formalanalysis}{Formal analysis}
\DeclareTranslation{Spanish}{formalanalysis}{Análisis formal}
\DeclareTranslation{French}{formalanalysis}{Analyse formelle}
\DeclareTranslation{German}{formalanalysis}{Formale Analyse}
% FUNDING ACQUISITION
\DeclareTranslation{Portuguese}{funding}{Aquisição de financiamento}
\DeclareTranslation{English}{funding}{Funding acquisition}
\DeclareTranslation{Spanish}{funding}{Adquisición de financiamiento}
\DeclareTranslation{French}{funding}{Obtention du financement}
\DeclareTranslation{German}{funding}{Förderung-Akquisition}
% INVESTIGATION
\DeclareTranslation{Portuguese}{investigation}{Investigação}
\DeclareTranslation{English}{investigation}{Investigation}
\DeclareTranslation{Spanish}{investigation}{Investigación}
\DeclareTranslation{French}{investigation}{Recherche}
\DeclareTranslation{German}{investigation}{Untersuchung}
% METHODOLOGY
\DeclareTranslation{Portuguese}{methodology}{Metodologia}
\DeclareTranslation{English}{methodology}{Methodology}
\DeclareTranslation{Spanish}{methodology}{Metodología}
\DeclareTranslation{French}{methodology}{Méthodologie}
\DeclareTranslation{German}{methodology}{Methodik}
% PROJECT ADMINISTRATION
\DeclareTranslation{Portuguese}{projadm}{Administração de projetos}
\DeclareTranslation{English}{projadm}{Project~administration}
\DeclareTranslation{Spanish}{projadm}{Administración de proyectos}
\DeclareTranslation{French}{projadm}{Administration du projet}
\DeclareTranslation{German}{projadm}{Projektverwaltung}
% RESOURCES
\DeclareTranslation{Portuguese}{resources}{Recursos}
\DeclareTranslation{English}{resources}{Resources}
\DeclareTranslation{Spanish}{resources}{Recursos}
\DeclareTranslation{French}{resources}{Fourniture de ressources}
\DeclareTranslation{German}{resources}{Ressourcen}
% SOFTWARE
\DeclareTranslation{Portuguese}{software}{Programas}
\DeclareTranslation{English}{software}{Software}
\DeclareTranslation{Spanish}{software}{Software}
\DeclareTranslation{French}{software}{Développement informatique}
\DeclareTranslation{German}{software}{Software}
% SUPERVISION
\DeclareTranslation{Portuguese}{supervision}{Supervisão}
\DeclareTranslation{English}{supervision}{Supervision}
\DeclareTranslation{Spanish}{supervision}{Supervisión}
\DeclareTranslation{French}{supervision}{Supervision}
\DeclareTranslation{German}{supervision}{Supervision}
% VALIDATION
\DeclareTranslation{Portuguese}{validation}{Validação}
\DeclareTranslation{English}{validation}{Validation}
\DeclareTranslation{Spanish}{validation}{Validación}
\DeclareTranslation{French}{validation}{Validation}
\DeclareTranslation{German}{validation}{Validierung}
% VISUALIZATION
\DeclareTranslation{Portuguese}{visualization}{Visualização}
\DeclareTranslation{English}{visualization}{Visualization}
\DeclareTranslation{Spanish}{visualization}{Visualización}
\DeclareTranslation{French}{visualization}{Visualisation}
\DeclareTranslation{German}{visualization}{Visualisierung}
% WRITING
\DeclareTranslation{Portuguese}{writing}{Escrita~-- rascunho original}
\DeclareTranslation{English}{writing}{Writing~-- original draft}
\DeclareTranslation{Spanish}{writing}{Redacción~-- borrador original}
\DeclareTranslation{French}{writing}{Rédaction~-- version originelle}
\DeclareTranslation{German}{writing}{Schreiben~-- Originalentwurf}
% REVIEW
\DeclareTranslation{Portuguese}{review}{Escrita~-- revisão e edição}
\DeclareTranslation{English}{review}{Writing~-- review and editing}
\DeclareTranslation{Spanish}{review}{Redacción~-- Revisión y edición}
\DeclareTranslation{French}{review}{Rédaction~-- Révision et correction}
\DeclareTranslation{German}{review}{Schreiben~-- Review und Bearbeiten}
% Authors contributions END
% NOTE
\DeclareTranslation{Portuguese}{note}{Nota: }
\DeclareTranslation{English}{note}{Note: }
\DeclareTranslation{Spanish}{note}{Nota: }
\DeclareTranslation{French}{note}{Remarque: }
\DeclareTranslation{German}{note}{Hinweis: }
% SOURCE
\DeclareTranslation{Portuguese}{source}{Fonte: }
\DeclareTranslation{English}{source}{Source: }
\DeclareTranslation{Spanish}{source}{Fuente: }
\DeclareTranslation{French}{source}{Source: }
\DeclareTranslation{German}{source}{Quelle: }


%
%\DeclareTranslation{Portuguese}{}{}
%\DeclareTranslation{English}{}{}
%\DeclareTranslation{Spanish}{}{}
%\DeclareTranslation{French}{}{}
%\DeclareTranslation{German}{}{}

